Behavioural Types for Memory and Method Safety in a Core Object-Oriented Language

We present a type-based analysis ensuring memory safety and object protocol completion in the Java-like language Mungo. Objects are annotated with usages, typestates-like specifications of the admissible sequences of method calls. The analysis entwines usage checking, controlling the order in which methods are called, with a static check determining whether references may contain null values. The analysis prevents null pointer dereferencing and memory leaks and ensures that the intended usage protocol of every object is respected and completed. The type system has been implemented in the form of a type checker.

==> article/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

A central notion in imperative programming is that of a
\emph{reference} because it underpins the implementation of data
structures: elements of a composite data structure can be retrieved by
following a reference where \emph{null-pointers} (or null-references)
are used to represent endpoints of a data structure such as leaves of
a tree or empty lists.
%
Object-oriented programming is often an extension of the imperative
paradigm, and the notion of references (and null-pointers) is central
to the implementation of objects as well. Programs written in this
paradigm are particularly prone to the problem of \emph{null-pointer
  dereferencing}~\cite{Hoare} (or simply null dereferencing), and the
situation is further complicated by the possibility of aliasing, that
is, if the same resource can be referred to by different names.
%
Sunshine~\cite[Table 1.1]{SunshineAldrich} analyses the questions
posted to StackOverflow referring to one of the \texttt{java.lang}
exception types and notes that, as of 1 November 2013, the most common
exception was that of null dereferencing.
%
Another problem that occurs in object-oriented programming is that of
run-time errors caused by incorrect method calls: a method call to an
object $o$ can fail, either because the method does not exist at all
in $o$ or is simply not available at present.
% The former error can occur at run-time, since object references can change during program execution, and the 
The latter error can occur at run-time, since some methods are only meaningful in certain program states. For instance, we should not be able to call a \textsf{read} method on a file object that has not been opened yet.

\subsection{The curse of null-dereferencing and incorrect method calls}
%
The problem of null-pointer dereferencing is of great importance. Meyer~\cite{DBLP:journals/cacm/Meyer17} writes 
\begin{quote}
  \textsl{
  Talking about sources of crashes, one of the principal plagues of
  modern programs is null-pointer dereferencing. This term denotes
  what happens when you call $x.f$, meaning apply $f$ (a field access
  or an operation) to the object that $x$ references. \ldots But then
  you should make sure that $x.f$ never gets called for null $x$,
  since there is in that case no object to which we can apply $f$.
  %
  The problem is particularly acute in object-oriented programming
  languages, where $x.f$ is the major computational mechanism. \ldots
  %
  % Every single execution of this construct (how many billions of them occurred in running programs around the world since you started reading this article?) faces that risk. \ldots
  %
  This fundamental brittleness threatens the execution of most programs running today. Calling it a "billion-dollar mistake" \ldots  is not an exaggeration.
  }
\end{quote}

% Moved it here...
%
% There are various solutions to this problem that rely on statically checking for null-pointer dereferencing. 
% %
% For instance, the type system of Eiffel \cite{DBLP:journals/cacm/Meyer17} distinguishes between attached and detachable types: variables of an attached type can never be assigned to a void value; this is only allowed for variables of detachable type. Other, more recent approaches use notions of behavioural types that describe the usage protocols that must be followed by fields and methods in an object. 

Existing approaches for preventing null-dereferencing require annotations, either in the form of pre-conditions or type qualifiers. 
%
F\"{a}hndrich and Leino \cite{Fahndrich2003} use type qualifiers together with a data flow analysis to determine if fields are used in a safe manner, while Hubert \emph{et al.}
% , Jensen and Pichardie 
rely on a constraint-based flow analysis \cite{hubert2008}. 
%
The fact that these approaches rely on the programmer could be viewed as a limitation, as they do not ensure the absence of null  dereferencing "for free" in well-typed programs. 
%
Recently, the type system of Eiffel \cite{DBLP:journals/cacm/Meyer17} has been extended to distinguish between attached and detachable types: variables of an attached type can never be assigned to a void value; this is only allowed for variables of detachable type.
%
Alternatively, static analysis tools could be used to check the code
once it is in a stable state, but including the analysis in the type
system lifts the burden from the programmer since there is no longer a
need for additional annotations or extra tools.

In this work, we note that the interplay between null dereferencing
and the \emph{order} in which methods of an object are invoked is
important. This is the case, since the execution of a method body will
typically change the program state and can cause fields of an object
to become nullified.
%
A recent manifestation of this is the bug found found in Jedis
\cite{jedis1}, a Redis \cite{redis1} Java client. In essence, the
problem was that a \textsf{close} method could be called even after a
socket had timed out \cite[Issue 1747]{jedis1}.   
%
Bugs related to calling methods in an unintended order are hard to
find: Jedis was launched in 2011 and the bug was found in 2018.  
%
However, it is normal to assume that methods should be called
according to a specific protocol: for instance, in an iterator one
should call \textsf{hasNext} before calling \textsf{next}. 

\subsection{Behavioural types} 

Behavioural types have been used to formalise the \emph{inter-method} information described above: an object follows a protocol that describes the \emph{admissible sequences of method invocations}, and behavioural types are used for describing such object protocols. For surveys of the foundations of behavioural types and their use in programming languages, see \cite{HuttelEtal,AnconaEtal}

Here we distinguish between two major approaches to behavioural type
systems. The notion of \emph{typestates} has its origin in the work by
Strom and Yemini \cite{StromYemini}; the idea is to annotate the type
of an object with information pertaining to its current state. Later
work includes that of Vault \cite{DBLP:conf/pldi/FahndrichD02}, Fugue
\cite{DBLP:conf/ecoop/DeLineF04} and the work by Aldrich \emph{et al.}
on Plaid \cite{plaid,DBLP:conf/oopsla/SunshineSNA11}. Garcia \emph{et
  al.} describe a gradual typestate system \cite{GarciaEtal} that
integrates access permissions with gradual types
\cite{DBLP:conf/ecoop/SiekT07} to control aliasing in a more robust
way. There appears to have been little work on memory safety; work by
Suenaga et al. \cite{Suenaga:2012:TSR:2398857.2384618,Suenaga:2016}
studies behavioural type systems for memory deallocation in an
imperative language without objects.
%
Another approach taken is that of \emph{session types}
\cite{Honda}. This line of work originated in the setting of the
$\pi$-calculus and type systems for describing the protocol followed
by named channels in a $\pi$-calculus process. Here, the session type
of a channel is a protocol that describes the sequence of
communications that the channel must be involved in. A session channel
is linear: it will only be used once with the given protocol, and its
protocol evolves as the result of each communication that it is
involved in.
%
The work by Gay \emph{et al.} \cite{GayEtal} is a meeting of these two
approaches; the type of a class $C$ is annotated with a \emph{usage}
whose typestate that describes the protocol that must be followed by
any object that is an instance of $C$. In other words, the usage of an
object is a session that the object must follow. It is this work that
is the outset of the present paper.

\subsection{The importance of session completion} 
\label{sec:session-complete}

All the behavioural type systems that have been proposed for
object-oriented programming come with a \emph{fidelity} result,
guaranteeing that the actual sequences of method calls for any object
will follow those specified by the behavioural type of the object. 
%
However, session fidelity, by itself, is not enough to ensure the
absence of null dereferencing. A stronger requirement in the form of
\emph{protocol completion} is necessary: A well-typed program will
never leave the protocol incomplete by losing a reference to an object
at some point during its execution.
%
The two issues are in fact \emph{interdependent}: the tracking of
null-references via a \emph{linear type discipline} is essential for
guaranteeing the completion of a (behavioural type) protocol of an
object.

Consider the class declaration \textsf{File} in Listing \ref{listing:file1}.
%
A potential run-time error is that a user of this class can close a file that had not been opened; another is that files can be left open at the end of execution. 
%
\lstset{escapeinside={(*@}{@*)}}
\begin{lstlisting}[label={listing:file1},caption={An example class describing files},firstnumber=9]  

class File {
    // u1 = {open;<rec X.{neof;<{read;X}, {close;end}>},end>} (*@\label{lst:code:4}@*)
    
    bool open(){...}
    bool neof(){...}
    char read(){...}
    void close(){...}
  }
\end{lstlisting}
%
In order to prevent this, we can annotate the class with a method
usage describing the protocol, as shown on line \ref{lst:code:4},
followed by instances of the object and insist that this protocol must
be carried out to completion. But in order to achieve this, both
methods and \emph{fields} should obey their associated
protocols. Within any instance of a class, its fields must be used
correctly so as to ensure that their usage protocol is observed and
executed to completion, whereas method must be invoked in the expected
usage order until completion; to attain this, avoiding field null
dereferencing is crucial. See Listing \ref{listing:file2}.
 %
%  This requires additional annotation as shown for class \textsf{FileReader} below.
% 
 \lstset{escapeinside={(*@}{@*)}}
 \begin{lstlisting}[label={listing:file2},caption={An example class
     intended for reading files},firstnumber=9]
  class FileReader {
      // u2={init;{purge;{getSize;end} + getSize;end}}   (*@\label{lst:code:0}@*)
      
    File f;  int size;
    void init() {
     f = new File(); (*@\label{lst:code:1}@*)
     size = 0; (*@\label{lst:code:3}@*)
    }
    void purge() {
     if (f.open()) {
       while (f.neof()) {f.read();size = size + 1;}
       f.close();(*@\label{lst:code:2}@*)
    }
    int getSize() { size; }
  }
\end{lstlisting}
%
The usage information \textsf{u2} on line \ref{lst:code:0} for objects
of class \textsf{FileReader} requires that the \textsf{init()} method
is called first, followed either by the call sequence \textsf{purge()}
and \textsf{getSize()} or else by simply invoking \textsf{getSize()}.
%
Importantly however, it must also use objects of type \textsf{File}
with usage information \textsf{u1} on line\ref{lst:code:4}, stating
that after it is opened, a \textsf{File} object can be checked whether
it has reached its end-of-file: if so it can only be closed, else it
can be read and then checked for end-of-file again.
%
 %COVER ALL FOUR KINDS OF ERRORS.
%
Stated otherwise, we have to understand how these requirements can
live together. Below is a list of potential causes of error that
existing behavioural-type solutions for objects do not handle:
\begin{itemize}
\item A program that adheres to program fidelity allows us to omit
  line \ref{lst:code:1} that initialises field \textsf{f} with a new
  \textsf{File} object.  However, calling \textsf{read()} on field
  \textsf{f} in method \textsf{purge()}, even if we follow the
  prescribed protocol \textsf{u2} and invoke \textsf{init()} first,
  would result in a null-pointer dereferencing. This is an example of
  how the order in which methods are invoked can impact on the
  possibility of null-dereferencing.
\item Similarly, session fidelity also allows us to add the command
  \lstinline{f = null} at line \ref{lst:code:3} before calling
  \lstinline{size = 0}.  This would result in losing the reference to
  the object, breaking linearity.
\item Session fidelity also permits us to add the command \lstinline{f = new File()} at line\ref{lst:code:2} before calling
  \lstinline{close()}.  Again, this would result in us losing the
  reference to the previous object stored in field \textsf{f} that has
  not yet completed its protocol \textsf{u1}.
\end{itemize}

A crucial observation is that usages are vital for permitting a
\emph{finer} analysis that guarantees the absence of null
dereferencing that is also \emph{compositional}. Stated otherwise, our
proposed analysis provides such guarantees for programs following the
intended usage protocols. Moreover, we are able to do so by analysing
the source code of each individual class \emph{in isolation}. This
allows our type analysis to accept more code (\emph{e.g.} in general,
any standard null dereference analysis for class \textsf{FileReader}
without any usage analysis would fail).
  
\subsection{A core Java with behavioural types}
\label{sec:mungo}
%
Our study is cast within the \mungo and \stmungo tool suite \cite{KouzapasEtal} that consider a subset of Java. It is developed at the University of Glasgow and is based on versions of the type system of Gay et al. \cite{GayEtal}. 
%
In \mungo, objects are used according to a linear type discipline -- an object can be written to and subsequently read at most once which in turn control aliasing and permits compositional reasoning via the type system. 
%
This approach 
% is similar to the linear usage of channels in session type theory. It 
makes it possible to verify properties such as the adherence to the prescribe object usage by means of static type-checking, i.e. \emph{session fidelity}.  However, the existing tool suite does not provide guarantees for protocol completion or null dereferencing.  
% as discusseda prescribed object usage protocol does not necessarily need not be associated to the actual run-time behaviour of the program, and as a consequence, certain run-time errors may still crop up even when this protocol is observed.


\subsection{Generic classes in \mungo}
\label{sec:generic-mungo}

Previous work on \mungo \cite{KouzapasEtal} has not considered
composite data, but for the analyses proposed to be useful for more
substantial fragments of Java, this should be dealt with. In the
present work we go some way towards a treatment of data structures by
introducing a simple notion of generic classes that avoids the
problems with unsoundness reported by Amin and Ross \cite{Amin2016}.

An example of a program using our notion generic classes can be seen
below. The program uses a version of the identity function $f(x)=x$
written in an object oriented setting. The \texttt{Id} class is a
generic class that can be instantiated with a type parameter and
provides a \texttt{id} method that works for that type. Here, $\alpha$
is a class type variable and $\beta$ is a usage variable. The class
can therefore be instantiated for \emph{any} class $\alpha$ and
\emph{any} usage $\beta$.

\begin{lstlisting}
class$\<\alpha[\beta]\>$ Id {
    $\U$ = {id ; end}
    $\alpha[\beta]$ id($\alpha[\beta]$ x) { x }
}
[...]
// Use of class
b = new Boolean; // A class with usage $\U$={setVal;{getVal;end}}
b.setVal(true);
f = new Id$\<$Boolean[{getVal;end}]$\>$;
l = f.id(b)
\end{lstlisting}

This type of generics, where no bounds are placed on the type
parameters, can model the classes in Java that extend the
\texttt{java.util.Collection} interface, such as \texttt{ArrayList},
\texttt{ArrayDequeue} and \texttt{HashSet}, which all work for all
type parameters.


\subsection{Contributions} \label{subsec:errors}
%

In this paper we present the first (to our knowledge) behavioural type system for the realistic object-oriented language \mungo, that rules out null dereferencing and memory leaks as a by-product of a
% safety property -- protocol fidelity -- and of a 
(weak) liveness property -- object protocol completion for terminated programs. 
% Besides the usual guarantees (absence of \emph{message-not-understood} errors), protocol fidelity is an expected property in behavioural type systems, but these do not usually guarantee, for mainstream like languages, protocol completion and none has until now ensured memory safety (no \emph{null-pointer dereferencing} nor \emph{memory leaks}).
%
Moreover we extend the \mungo language of \cite{KouzapasEtal} with a notion of generics that is similar to parametric polymorphism. However, unlike the type system of Java \cite{Amin2016} the version of generic classes presented here does not prevent the type system from being sound. 
%
% %
% This paper extends the results of \mungo by presenting a type-based analysis that is able to analyze both method usage and null pointer dereferencing and related errors. 
%
In our analysis, every field can be written to and subsequently read \emph{at most once}. Strictly speaking, access is therefore affine, since fields that are never assigned to or read from will of course not cause any problems.
%
Every method of an object must adhere to a \emph{usage} behaviour that describes the admissible sequences of method calls. 

Overall, our type system prevents four kinds of errors related to method, field, and parameter access. The first kind is standard in object-oriented programming:
%
\begin{description}
\item[Method not understood]: 
% This kind of error occurs if 
the method
  $m$ in object $o$ does not exist at all.
\item[Field not understood:] 
% This kind of error occurs if 
the field
  $f$ in object $o$ does not exist at all.
\end{description}

The second kind is specific to behavioural type systems:
%
\begin{description}
\item[Method not available:] 
% This kind of error occurs if 
the method
  $m$ in object $o$ exists but cannot be called in the object's state.
\end{description}

The third kind is a contribution of the present paper, namely that of preventing null dereferencing:
%
\begin{description}
\item[Field not available:] 
% This kind of error occurs if 
the field $f$ exists in object $o$ but is not available, in the sense that accessing it could cause a null dereferencing.
\item[Parameter not available:] 
% This kind of error occurs if 
the parameter $x$ exists in method $m$ but is not available, in the sense that  accessing it could cause a null dereferencing.
\end{description}

The fourth kind is also a contribution of the present paper, that of preventing memory leaks leading to the failure to complete an object protocol:
%
\begin{description}
\item[Field misused:] 
% This kind of error occurs if 
the field $f$ in object $o$ containing an object reference $o'$ is rewritten before the completion of the latter object protocol.
\item[Parameter misused:] 
% This kind of error occurs if 
the parameter $x$ of method $m$ containing an object reference $o$ is rewritten or not returned before the completion of the latter object protocol.
\end{description}

The main result for our type system is that of type safety: If a program is well-typed, it will not exhibit any of these four kinds of errors.  The rest of this paper is structured as follows. In Section \ref{sec:syntax} we introduce the syntax of the \mungo language. In Section \ref{sec:semantics} we present the operational semantics of \mungo. In Section \ref{sec:typesystem} we present the type system, and in Section \ref{sec:results} we present the soundness results concerning the type system.

% \textbf{Issues: 
% \begin{enumerate}
%     \item What we should say is that we do not leave the protocol incomplete by loosing a reference to an object half-way through its protocol.
%     \item inconsistent terminology regarding linearity. \S\ref{sec:session-complete} and \S\ref{sec:mungo}.
%     \item \S\ref{sec:generic-mungo} is neither here nor there. One idea could be to move it to the body sections.
%     \item In \S\ref{sec:generic-mungo} $\alpha[\beta]$ is obscure.  We should instead change the existing main example.
%     \item say that we show that the technique is compatible with generics (and this is why we extend the Mungo Language, to be able to show this).    
%     % \item I could only see three kinds of errors in \S\ref{subsec:errors}.
%     \item Have a small example of usage transitions (referring to the example in Section 1) at the end of Section 2.
%     \item Small examples in Section 4 concerning the type rules for class definition (Table 6, TCBR) and method invocations (Table 8, TCALLF).
%     \item Explain why envTf must be terminated in Table 7.
%     \item Leave out the lemmas in Section 5, if we need more space.
% \end{enumerate}
% }

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> article/proofs/preservation_objects.tex <==
\begin{lemma}{(Preservation of object types.)}
If $\Lambda;envT_O, o \mapsto t \cdot envT_S \vddash e : t' \triangleright \Lambda';envT_O, o\mapsto C\<t''\>[\U]\cdot envT_S$ then $t = C\<t''\>[\U']$.

\end{lemma}
\begin{proof}
We proceed by induction on the structure of the derivation for expression type judgements. Only the rules \rt{TCallO}, \rt{TSwO} and \rt{TObj} can update the bindings in $envT_O$.

We see that \rt{TObj} cannot have been used to conclude the hypothesis, since if it were used, we would have $o\not\in\dom{envT_O}$, which contradicts our assumption.

If \rt{TCallO} was used, then our hypothesis is:
$\Lambda;envT_O, o \mapsto t \cdot envT_S \vddash o.m(e) : t' \triangleright \Lambda';envT_O, o\mapsto C\<t''\>[\U]\cdot envT_S$. From the hypothesis we know $\Lambda;envT_O, o\mapsto t \cdot envT_S \vddash e : t''' \triangleright \Lambda';envT_O', o \mapsto C\<t''\>[\U'] \cdot envT_S'$. By IH we have that $t = C\<t''\>[\U'']$.

If \rt{TSwO} was used, then our hypothesis is:
$\Lambda;envT_O, o \mapsto t \cdot envT_S \vddash \sf{switch}\ (o.m(e))\ \{l_i : e_i\}_{l_i \in L} : t' \triangleright \Lambda';envT_O, o \mapsto C\<t''\> \cdot envT_S$. And from the premise of \rt{TSwO} we get $\Lambda; envT_O, o \mapsto t\cdot envT_S \vddash o.m(e) : L \triangleright \Lambda''; envT_O'', o \mapsto C\<t''\>[(\<l_i : u_i\>_{l_i \in L})^{\vv{E}}] \cdot envT_S''$. By IH we have that $t=C\<t''\>[\W]$.

\end{proof}

==> article/proofs/preservation_parameter.tex <==
\begin{lemma}{(Preservation of parameter types.)}
\label{lemma:preservation-for-parameters}
If $\Lambda;\Delta\cdot(o, [x \mapsto t]) \vddash e : t' \triangleright \Lambda';\Delta' \cdot (o, \mapsto C\<t''\>[\U])$ then $t = C\<t''\>[\U']$.

\end{lemma}
\begin{proof}
We proceed by induction on the structure of the derivation for expression type judgements. The following rules uses the parameter binding of $x$: \rt{TLinPar}, \rt{TNoLPar}, \rt{TCallP} and \rt{TSwP}. 

We see that \rt{TLinPar} could not have been used to conclude the hypothesis, since the resulting parameter binding is different from $\bot$. Similarly \rt{TLinFld} could not have been used, since the resulting type is not unrestricted. 

If \rt{TCallP} was used to conclude the hypothesis, we know that $\Lambda;\Delta \cdot (o, [x \mapsto t]) \vddash x.m(e) : t' \triangleright \Lambda';\Delta'\cdot(o, x \mapsto C\<t''\>[\U])$.  From the premise we know $\Lambda;\Delta \cdot (o, [x \mapsto t]) \vddash e : t'' \triangleright \Lambda'';\Delta''\cdot(o, x \mapsto C\<t''\>[\U''])$ then by IH we know that $t=C\<t\>[\U']$.

If \rt{TSwP} was used to conclude the hypothesis, we know that $\Lambda;\Delta \cdot (o, [x \mapsto t]) \vddash \sf{switch}\ (x.m(e))\ \{l_i : e_i\}_{l_i \in L} : t' \triangleright \Lambda';\Delta'\cdot(o, x \mapsto C\<t''\>[\U])$. From the premise of \rt{TSwP} we get that $\Lambda;\Delta \cdot (o, [x \mapsto t]) \vddash x.m(e) : L \triangleright \Lambda'';\Delta''\cdot(o, x \mapsto C\<t''\>[\U''])$. From IH we can then conclude that $t=C\<t\>[\U']$.
\end{proof}

==> article/proofs/strengthening.tex <==
\begin{lemma}{Strengthening for parameter bindings}

If $\Lambda;\Delta \cdot (o, [x\mapsto t']) \vddash e : t \triangleright \Lambda';\Delta' \cdot (o, [x \mapsto t''])$ and $x\not\in \fv(e)$ then $\Lambda;\Delta\cdot(o, \varepsilon) \vddash e : t \triangleright \Lambda';\Delta'\cdot (o, \varepsilon)$ 

\end{lemma}
\begin{proof}
Proof by induction on the structure of the derivation for expression type judgements. 

We look to the cases where the parameter binding of $x$ is used. This is the case in \rt{TLinPar}, \rt{TNoLPar}, \rt{TCallP}. However, to apply one of these rules, we must have that $x\in\fv(e)$, which by our hypothesis is a contradiction. Thus we can conclude that $\Lambda;\Delta \cdot (o, [x\mapsto t']) \vddash e : t \triangleright \Lambda';\Delta' \cdot (o, [x \mapsto t''])$ must have been concluded without using any of those rules, hence the parameter binding of $x$ has no influence on the result, and that $\Lambda;\Delta\cdot(o, \varepsilon) \vddash e : t \triangleright \Lambda';\Delta'\cdot (o, \varepsilon)$.
\end{proof}

==> article/proofs/substitution_continue.tex <==
\begin{lemma}{Substitution lemma for continue expressions.}
\label{lemma:substitution-continue}
Suppose $\Lambda;\Delta \vddash^{\Omega} e : t \triangleright \Lambda'; \Delta'$ and $\Lambda;\Delta \vddash^{\Omega'} e' : \sf{void} \triangleright \Lambda;\Delta$. Then $\Lambda;\Delta \vddash^{\Omega''} e\{k : e'/\sf{continue} \ k\} : t \triangleright \Lambda';\Delta'$.
\end{lemma}
% \begin{proof}
% We proceed by induction on the structure of the derivation for $\Lambda;\Delta \vddash^{\Omega} e : t \triangleright \Lambda'; \Delta'$. In this proof we only include the rules relevant for typing continue expressions.

% For the case \rt{TCon} it is only necessary to inspect the case where the labels match, $\Lambda;\Delta\vddash^{\Omega} \sf{continue}\ k : \sf{void} \triangleright \Lambda;\Delta$. Otherwise nothing will be replaced, and the case will be trivial. From the premise we have that $\Omega(k)=(\Lambda,\Delta)$, hence we know that $\Omega'=\Omega, k : (\Lambda;\Delta) = \Omega$. From the hypothesis we can then conclude that $\Lambda;\Delta \vddash^{\Omega'} e : \textsf{void} \triangleright \Lambda;\Delta$. Both premises of \rt{TLab} is then fulfilled, and we can conclude that $\Lambda;\Delta\vddash^{\Omega} \sf{continue}\ k \substitute{k : e'}{\sf{continue}\ k} : \sf{void} \triangleright \Lambda;\Delta$.

% For the case \rt{TLab}. Assume $\Lambda;\Delta\vddash^{\Omega} k' : e : \sf{void} \triangleright \Lambda;\Delta$ and $\Lambda;\Delta \vddash^{\Omega} e' : \sf{void} \triangleright \Lambda;\Delta$. From the premise of \rt{TLab} we have $\Omega'=\Omega, k' : (\Lambda;\Delta)$ and $\Lambda;\Delta\vddash^{\Omega'}e:\sf{void} \triangleright \Lambda;\Delta$. By IH we have $\Lambda;\Delta \vddash^{\Omega'} e\substitute{k:e'}{\sf{continue}\ k} : \sf{void} \triangleright \Lambda;\Delta$. But then directly we have $\Lambda;\Delta\vddash^{\Omega} k' : e\substitute{k:e'}{\sf{continue}\ k} : \sf{void}\triangleright \Lambda;\Delta$
% \end{proof}

==> article/proofs/substitution_parameters.tex <==
\begin{lemma}{Substitution lemma for parameters}
The lemma is split into three cases:
\begin{enumerate}
    \item If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t']) \vddash e : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto t''])$, $\Lambda, envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash v : t' \triangleright \_;\_$, $v\not\in \sf{objects}(e)$ and either $t'' = C[\U]$ or $t'' = \alpha[\beta]$ then $\Lambda; envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash e\{v / x\} : t \triangleright \Lambda'; envT_O', v \mapsto t'' \cdot envT_S' \cdot (o, \varepsilon)$. 
    \item If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto b]) \vddash e : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto t''])$ and $\Lambda; envT_O \cdot envT_S \cdot (o, \varepsilon) \vddash v : b \triangleright \_;\_$ then $\Lambda; envT_O \cdot envT_S \cdot (o, \varepsilon) \vddash e\{v / x\} : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, \varepsilon)$
    \item If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t']) \vddash e : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto \bot])$, $\Lambda, envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash v : t' \triangleright \_;\_$, $v\not\in \sf{objects}(e)$ then $\Lambda; envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash e\{v / x\} : t \triangleright \Lambda'; envT_O \cdot envT_S' \cdot (o, \varepsilon)$. 
\end{enumerate}
\end{lemma}
\begin{proof}
We proceed by using induction on the structure of type judgements for expressions. In this proof we only look at relevant type rules for each case of the substitution lemma.

Case 1:
\begin{description}

    \item[\rt{TNoLPar \& TLinPar}]
    We cannot use rule \rt{TNoLPar} because in our assumptions we have that $t'$ is a class type from lemma \ref{lemma:preservation-for-parameters}, hence the premise of \rt{TNoLPar} $\neg \lin(t')$ is not fulfilled. Additionally, rule \rt{TLinPar} also cannot have been used since $t'' \neq \bot$ which is not the case based on our assumptions, and using \rt{TLinPar} results in the parameter $x$ being mapped to $\bot$.
    
    \item[\rt{TCallP}]
    From \rt{TCallP} we know $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t^{(4)}]) \vddash x.m(e) : t' \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto C\<t''\>[\mathcal{W}]])$, $\mathcal{U} \trans[m] \mathcal{W}$, and $t' \ m(t \ x) \in C\<t''\>.\sf{methods}$.
    
    We now have to show:
    \begin{multline}
    \label{eq:substitution-tcallp-case-1-3}
        \Lambda;envT_O, v \mapsto C\<t''\>[\mathcal{U}] \cdot envT_S \cdot (o, \varepsilon) \vddash \\ x.m(e)\{v / x\} : t \triangleright \Lambda';envT_O', v \mapsto C\<t''\>[\mathcal{W}] \cdot envT_S' \cdot (o,\varepsilon)
    \end{multline}
    
    We can type \eqref{eq:substitution-tcallp-case-1-3} using \rt{TCallO}.
    
    From the induction hypothesis we have:
    \begin{multline}
    \label{eq:substitution-tcallp-case-1-4}
        \Lambda;envT_O,v \mapsto t^{(4)} \cdot envT_S \cdot (o, \varepsilon) \vddash \\ e\{v / x\} : t \triangleright \Lambda'; envT_O', o \mapsto C\<t''\>[\mathcal{U}] \cdot envT_S' \cdot (o,\varepsilon) 
    \end{multline} and from our assumptions we have that $\mathcal{U} \trans[m] \mathcal{W}$ and $t' \ m(t \ x) \in C\<t''\>.\sf{methods}$. We can know conclude \eqref{eq:substitution-tcallp-case-1-3} is correct since the premises of \rt{TCallO} are fulfilled from our assumptions and \eqref{eq:substitution-tcallp-case-1-4}. 
    
    \item[\rt{TSwP}]
    From \rt{TSwP} we know $\Lambda;envT_O \cdot envT_S \cdot (o, [x \mapsto t^{(4)}]) \vddash \\ \sf{switch}(x.m(e)) \{l_i : e_i\}_{l_i \in L} : t' \triangleright \Lambda';envT_O' \cdot envT_S' \cdot (o, [x \mapsto t^{(5)}])$ and $t^{(5)} = C\<t\>[U]$.
    %\begin{multline}
    %\label{eq:substitution-tswp-case-1-2}
    %    \Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t^{(4)}]) \vddash \\ x.m(e) : L \triangleright \Lambda'';envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto C\<t\>[(\<l_i : u_i\>_{l_i \in L})^{\vv{E}}]])
    %\end{multline}
    %\begin{equation}
    %\label{eq:substitution-tswp-case-1-3}
    %    \forall i . \Lambda'';envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto C\<t\>[u_i^{\vv{E}}]]) \vddash e_i : t' \triangleright \Lambda';envT_O' \cdot envT_S' \cdot (o, [x \mapsto t^{(6)}])
    %\end{equation}
    
    We then have to show:
    \begin{multline}
    \label{eq:substitution-tswp-case-1-2}
        \Lambda;envT_O, o \mapsto t^{(4)} \cdot envT_S \cdot (o, [x, \varepsilon] \vddash \\ \sf{switch}(x.m(e))\{v / x\} : t \triangleright \Lambda';envT_O', o \mapsto t^{(5)} \cdot envT_S' \cdot (o, [x, \varepsilon])
    \end{multline}
    
    From our induction hypothesis we have
    \begin{multline}
    \label{eq:substitution-tswp-case-1-3}
        \Lambda; envT_O, o \mapsto t^{(4)} \cdot envT_S \cdot (o, [x, \varepsilon]) \vddash \\ x.m(e)\{v / x\} : L \triangleright \Lambda'';envT_O'',o \mapsto C\<t\>[(\<l_i : u_i\>_{l_i \in L})^{\vv{E}}] \cdot envT_S'' \cdot (o, \varepsilon)
    \end{multline}
    and
    \begin{multline}
    \label{eq:substitution-tswp-case-1-4}
        \forall i . \Lambda'';envT_O'', o \mapsto C\<t\>[u_i^{\vv{E}}] \cdot envT_S'' \cdot (o, [x, \varepsilon) \vddash \\ e_i (v / x) : t' \triangleright \Lambda';envT_O', o \mapsto t^{(5)} \cdot envT_S' \cdot (o, \varepsilon)
    \end{multline}
    
    We can now conclude \eqref{eq:substitution-tswp-case-1-2} is correct since the premises of \rt{TSwP} are fulfilled from \eqref{eq:substitution-tswp-case-1-3} and \eqref{eq:substitution-tswp-case-1-4}.
    
\end{description}

Case 2.

We assume $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto b]) \vddash e : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto t''])$ and $\Lambda; envT_O \cdot envT_S \cdot (o, \varepsilon) \vddash v : b \triangleright \_;\_$ 
    
then $\Lambda; envT_O \cdot envT_S \cdot (o, \varepsilon) \vddash e\{v / x\} : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, \varepsilon)$

\begin{description}
    \item[\rt{TLinPar}] 
    
    We cannot have used \rt{TLinPar} because from the premise we have $\lin(t)$ and we know $\neg \lin(b)$. Hence the rule cannot have been applied.
    
    \item[\rt{TCallP}]
    
    We cannot have used \rt{TCallP} because from the conclusion we have $\Lambda;\Delta\cdot(o,S) \vdash_{\vv{D}} x.m(e):t' \triangleright \Lambda';\Delta'\cdot(o,[x\mapsto C\<t''\>[\mathcal{W}]])$ and therefore $t'' = C\<t\>[W]$. From Lemma \ref{lemma:preservation-for-parameters}, we have that $\Lambda'; \Delta' \cdot (o, [x \mapsto C\<t^{(3)}\>[U]) \vddash e : t^{(4)} \triangleright \Lambda'; \Delta' \cdot (o, [x \mapsto C\<t^{(3)}\>[W])$, from this lemma we get that $b \neq c\<t\>[U]$. Hence the rule cannot have been applied. 
    
    \item[\rt{TSwP}]
    
    We cannot have used \rt{TSwP}. From the premise we have that $\Lambda; \Delta \cdot (o, S) \vddash x.m(e):L \triangleright \Lambda'';\Delta'' \cdot (o,[x \mapsto C\<t\>[(\<l_i :u _i\>_{l_i\in L})^{\vv{E}}]])$. From Lemma \ref{lemma:preservation-for-parameters}, we have that $\Lambda', \Delta' \cdot (o, [x \mapsto C\<t^{(3)}\>[U]) \vddash e : t^{(4)} \triangleright \Lambda', \Delta' \cdot (o, [x \mapsto C\<t^{(3)}\>[W])$, from this lemma we get that $b \neq c\<t\>[U]$. Hence the rule cannot have been applied. 
    
    \item[\rt{TNoLPar}]
    
    From \rt{TNoLPar} we have $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto b]) \vddash x:b \triangleright \Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto b])$ and $\neg \lin(b)$
    
    Show $\Lambda; envT_O \cdot envT_S \cdot (o, \epsilon) \vddash x \substitute{v}{x} :b \triangleright \Lambda; envT_O \cdot envT_S \cdot (o, \epsilon)$ and $\neg \lin(b)$
    
    From the definition of $\lin$ we have $\neg \lin(b)$. Conclude with \rt{TLit}, \rt{TVoid}, \rt{TBool} and \rt{TBot}. 

    \item[] Remaining rules follows directly from induction hypothesis. 

\end{description}

Case 3.

If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t']) \vddash e : t \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, [x \mapsto \bot])$, $\Lambda, envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash v : t' \triangleright \_;\_$, $v\not\in \sf{objects}(e)$ then $\Lambda; envT_O, v \mapsto t' \cdot envT_S \cdot (o, \varepsilon) \vddash e\{v / x\} : t \triangleright \Lambda'; envT_O \cdot envT_S' \cdot (o, \varepsilon)$. 

\begin{description}
\item [\rt{TLinPar}]

From \rt{TLinPar} we have $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t']) \vddash \triangleright x: t' \Lambda; envT_o \cdot envT_S \cdot (o, [x \mapsto \bot])$ and $\lin(t')$.

Show $\Lambda; envT_O, \{ v \mapsto t' \} \cdot envT_S \cdot (o, \epsilon) \vddash \triangleright x: t' \Lambda; envT_O \cdot envT_S \cdot (o, \epsilon)$. Conclude with \rt{TObj}.

\item [\rt{TSeq}]

From \rt{TSeq} we know $\Lambda; envT_O, envT_S \cdot (o, [x \mapsto t'']) \vddash e;e' :t' \triangleright \Lambda'; envT_O \cdot envT_S' \cdot (o, [x \mapsto \bot]) $

If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t'']) \vddash e : t \triangleright \Lambda'; envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto \bot])$
then by induction hypothesis we have
$\Lambda; envT_O, \{v \mapsto t''\}, envT_S \cdot (o, \epsilon) \vddash e \substitute{v}{x} : t \triangleright \Lambda''; envT_O'', envT_S'' \cdot (o, \epsilon)$ 
from induction hypothesis case 2 we have 
$\Lambda''; envT_O'', envT_S'' \cdot (o, \epsilon) \vddash e' \substitute{v}{x} : t' \triangleright \Lambda'; envT_O', envT_S' \cdot (o, \epsilon) $
hence premises are satisfied.

If $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t'']) \vddash e : t \triangleright \Lambda'; envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto t'''])$ and $t''' \neq \bot$ then by induction hypothesis case 1, we have
$\Lambda; envT_O \{v \mapsto t''\} \cdot envT_S \cdot (o, \epsilon) \vddash e\substitute{v}{x} : t \triangleright \Lambda''; envT_O'' \{v \mapsto t'''\} \cdot envT_S'' \cdot (o, \epsilon)$ and $\neg \lin(t)$
and by induction hypothesis we have 
$\Lambda''; envT_O'' \{v \mapsto t'''\} \cdot envT_S'' \cdot (o, \epsilon) \vddash e' \substitute{v}{x} \triangleright \Lambda'; envT_O' \cdot envT_S' \cdot (o, \epsilon)$
hence premises are satisfied.


\item [\rt{TIf}]

From \rt{TIf} we know $ \Lambda; envT_O, envT_S \cdot (o, [x \mapsto t'']) \vddash \sf{if}\ (e)\ \{e'\} \ \sf{else}\ \{e''\} :t' \triangleright \Lambda'; envT_O \cdot envT_S' \cdot (o, [x \mapsto \bot]) $

if $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t'']) \vddash e : \sf{bool} \triangleright \Lambda''; envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto \bot])$
then by induction hypothesis we have
$\Lambda; envT_O, \{v \mapsto t''\}, envT_S \cdot (o, \epsilon) \vddash e \substitute{v}{x} : \sf{bool} \triangleright \Lambda''; envT_O'', envT_S'' \cdot (o, \epsilon)$ 
and by induction hypothesis case 2 we have
$\Lambda''; envT_O'', envT_S'' \cdot (o, \epsilon) \vddash e' \substitute{v}{x} : t' \triangleright \Lambda'; envT_O', envT_S' \cdot (o, \epsilon) $ and 
$\Lambda''; envT_O'', envT_S'' \cdot (o, \epsilon) \vddash e'' \substitute{v}{x} : t' \triangleright \Lambda'; envT_O', envT_S' \cdot (o, \epsilon) $ 
hence the premise are satisfied.

if $\Lambda; envT_O \cdot envT_S \cdot (o, [x \mapsto t'']) \vddash e : \sf{bool} \triangleright \Lambda'; envT_O'' \cdot envT_S'' \cdot (o, [x \mapsto t'''])$ and $t''' \neq \bot$
then by induction hypothesis case 1 we have 
$\Lambda; envT_O,\{v \mapsto t''\} \cdot envT_S \cdot (o, \epsilon) \vddash e\substitute{v}{x} : \sf{bool} \triangleright \Lambda''; envT_O'', \{v \mapsto t'''\} \cdot envT_S'' \cdot (o, \epsilon)$ and $t''' \neq \bot$,
by induction hypothesis we have
$\Lambda''; envT_O''\{v \mapsto t'''\}, envT_S'' \cdot (o, \epsilon) \vddash e' \substitute{v}{x} : t' \triangleright \Lambda'; envT_O', envT_S' \cdot (o, \epsilon)$ and
$\Lambda''; envT_O''\{v \mapsto t'''\}, envT_S'' \cdot (o, \epsilon) \vddash e'' \substitute{v}{x} : t' \triangleright \Lambda'; envT_O', envT_S' \cdot (o, \epsilon)$
hence the premise are satisfied.

\end{description}
\end{proof}

==> article/proofs/type_preservation.tex <==
\begin{lemma}[Type preservation] Let $\vv{D}$ be such that $\vdash \vv{D}$ and let $\<h, env_S, e\>$ be a configuration. If $\vv{D} \vddash \<h, env_S, e\> \trans \<h', env_S', e'\>$ then:
\[
    \exists \Lambda, \Delta\ .\ \Lambda, \Delta \vddash \<h, env_S, e\> : t \implies \exists \Lambda^N, \Delta^N\ .\ \Lambda^N, \Delta^N \vddash \<h', env_S', e' \> : t
\]

\end{lemma}

\begin{proofsketch}
Inspection of the cases in the subject-reduction proof.
\end{proofsketch}

==> article/proofsummaries/subexpression_welltyped.tex <==
\begin{lemma}[Well-typedness of sub-configurations]
\label{lemma:subexpression_welltyped}

For any configuration $c$ on the following form:
\begin{itemize}
    \item $\<h, env_S, \sif{e}{e_1}{e_2}\>$
    \item $\<h, env_S, r.m(e)\>$
    \item $\<h, env_S, f = e\>$
    \item $\<h, env_S, e;e'\>$
    \item $\<h, env_S, \sf{switch}_{r.m}\ (e) \{l_i : e_i\}_{l_i \in L}\>$
\end{itemize}

We have that
%
\[\exists \Lambda, \Delta . \ \Lambda;\Delta \vddash c : t \triangleright \Lambda';\Delta' \implies \exists \Lambda''. \Delta''. \Lambda;\Delta \vddash \<h, env_S, e\> : t' \triangleright \Lambda'';\Delta''\]
\end{lemma}
\begin{proof}
We prove this result by a case analysis of the typing rules for expression used to show that the expression in the configuration is well typed. We show only a typical case here.

\begin{enumerate}[ncases]
    \item[\rt{FldC}]
    
    \begin{subproof}
    Assume that the configuration is well typed, that is: $\Lambda;\Delta\vddash\<h, env_S, f = e\> : \sf{void} \triangleright \Lambda'; \Delta'$, where $\Delta = envT_O \cdot envT_S$. 

All premises of \rt{WTC} can now be used as assumptions, since they must be satisfied for the configuration to be well-typed.

From \rt{TFld} we know $\Lambda;\Delta \vddash e : t \triangleright \Lambda\{o.f \mapsto t\};\Delta''\cdot(o, S)$. We can now show that $\Lambda;\Delta\vddash \<h, env_S, e\> : t \triangleright \Lambda\{o.f \mapsto t\};\Delta''\cdot(o, S)$ is a well typed configuration, by showing the premises of \rt{WTC}.

\begin{itemize}
    \item $\Lambda \vddash h$ follows from assumption
    \item $envT_S \vdash^h_e env_S$ follows from the premise of \rt{WTP-Fld} 
    \item $envT_O \vhdash e$, trivial since $\objects{f = e} = \objects{e}$, hence it follows from the assumptions.
    \item $\Lambda;\Delta \vddash e : t \triangleright \Lambda'\{o.f \mapsto t\};\Delta''\cdot(o, S)$ follows from \rt{TFld} as shown
    \item $\Lambda \vhdash \vv{D}$ follows from assumption
\end{itemize}
All premises of \rt{WTC} are satisfied for the sub-configuration, hence we can conclude $\Lambda;\Delta \vddash \<h, env_S, e\> : t \triangleright \Lambda'\{o.f \mapsto t\};\Delta''\cdot (o, S)$.

    \end{subproof}
\end{enumerate}
\end{proof}

\begin{lemma}[Well-typedness of return sub-configurations]
\label{lemma:subexpression_welltyped_return}

For a configuration $\<h, env_S \cdot (o, s), \return{e}\>$ we have that:

\[\exists \Lambda, \Delta . \ \Lambda;\Delta \cdot (o', S) \vddash \<h, env_S \cdot (o, s), return \{e\}\> : t \triangleright \Lambda';\Delta' \implies \exists \Lambda''. \Delta''.\Lambda;\Delta \vddash \<h, env_S, e\> : t \triangleright \Lambda';\Delta''\]
\end{lemma}
\begin{proof}

Assume $\Lambda;\Delta \cdot (o', S) \vddash \<h, env_S \cdot (o, s), \return{e}\> : t \triangleright \Lambda'; \Delta'$ where $\Delta = envT_O \cdot envT_S$. 

Similarly to the previous lemma, all premises of \rt{WTC} must be satisfied for the original configuration. Hence we can use the premises of \rt{WTC} in the proof for the sub-expression.

From \rt{WTP-Ret} we know that $o'=o$. Then from \rt{TRet} we know that $\Lambda;\Delta \vddash e : t \triangleright \Lambda'; \Delta''$. We can now show that $\Lambda;\Delta \vddash \<h, env_S, e\> : t \triangleright \Lambda'; \Delta''$.

\begin{itemize}
    \item $\Lambda \vddash h$ follows from assumption
    \item $envT_S \vdash^h_e env_S$ follows from premise of \rt{WTP-Ret}
    \item $envT_O \vhdash e$ is trivial since $\objects{\return{e}} = \objects{e}$, hence it follows from the assumptions.
    \item $\Lambda;\Delta \vddash e : t \triangleright \Lambda';\Delta''$ follows from \rt{TRet}
    \item $\Lambda \vhdash \vv{D}$ follows from assumption
\end{itemize}

Hence we have $\Lambda;\Delta \vddash \<h, env_S, e\> : t \triangleright \Lambda';\Delta''$.
\end{proof}

==> article/proofsummaries/weakening.tex <==



\begin{proof}
%The full proof can be found in Appendix \ref{app:weakening}. 
The proof proceeds by induction in the type rules. We highlight one case; the other cases are similar.

\begin{enumerate}[ncases]
    \item[\rt{TCallP}]
    \begin{subproof}
    \[\inference{\Lambda;\Delta \cdot (o, S) \vdash_{\vv{D}} e:t\triangleright \Lambda';\Delta' \cdot (o, [x\mapsto C\<t''\>[\mathcal{U}]]) & \mathcal{U}\trans[m] \mathcal{W} & \\ 
    t'\ m(t\ x')\{ e' \}\in C\<t''\>.\sf{methods}_{\vv{D}}}{\Lambda;\Delta\cdot(o,S) \vdash_{\vv{D}} x.m(e):t' \triangleright \Lambda';\Delta' \cdot (o,[x\mapsto C\<t''\>[\mathcal{W}]])}\]
    
    We assume that $\Lambda;\Delta\cdot(o,S) \vdash_{\vv{D}} x.m(e):t' \triangleright \Lambda';\Delta' \cdot (o,[x\mapsto C\<t''\>[\mathcal{W}]])$ is correct, $o'' \not\in \text{dom}(\Lambda)$ and $o^{(3)} \not\in \text{dom}(envT_O)$.
    
    We then show that:
    \begin{multline}
    \label{eq:tcallpweak-s}
        \Lambda, o'' \mapsto (C'\<t^N\>, envT_F); (envT_O, o^{(3)} \mapsto t^{(3)}) \cdot (o', S') \cdot envT_S \cdot(o,S) \vdash_{\vv{D}} x.m(e):t' \triangleright \\ \Lambda', o'' \mapsto (C'\<t^N\>, envT_F); (envT_O, o^{(3)} \mapsto t^{(3)}) \cdot (o', S') \cdot envT_S' \cdot(o,[x\mapsto C\<t''\>[\mathcal{W}]])
    \end{multline}
    
    From the induction hypothesis, we have that weakening lemma holds for the sub-expression $e$, hence both $\Lambda$ and $\Delta$ can be expanded while $e$ remains well-typed.
    
    The assumptions of \rt{TCallP} does not change, and we still have that $\U \trans[m] \W$ and $t'\ m(t\ x')\{ e' \}\in C\<t''\>.\sf{methods}_{\vv{D}}$.
    
    We can now conclude (\ref{eq:tcallpweak-s}), since all premises of \rt{TCallP} are satisfied. 
    \end{subproof}
\end{enumerate}
\end{proof}

==> article/titlepage.tex <==
\begin{titlepage}
\noindent
\begin{minipage}{.5\textwidth}
    \def\svgwidth{.9\textwidth}
    \input{image.pdf_tex}
\end{minipage}% This must go next to `\end{minipage}`
\begin{minipage}{.5\textwidth}
\flushright
  \textbf{Department of Computer Science}\\
  Aalborg University\\
  \url{http://cs.aau.dk}
\end{minipage}
\vspace{1cm}

\noindent
\begin{minipage}[t]{.48\textwidth}
    \vspace*{1cm}
    \noindent\textbf{Title:}\\ Soundness of the Mungo Type System with Generics\vspace*{0.4cm}

    \noindent\textbf{Theme:}\\ From Models to Reality\vspace*{0.4cm}
    
    \noindent\textbf{Project Period:}\\ Spring 2019\vspace*{0.4cm}
    
    \noindent\textbf{Group:}\\ D805F19\vspace*{0.4cm}
    
    \noindent\textbf{Participants:} \\Iaroslav Golovanov\\Mathias Jakobsen\\Mikkel Kettunen\vspace*{0.4cm}
    
    \noindent\textbf{Supervisor:}\\ Hans H\"uttel\vspace*{0.4cm}
    
    \noindent\textbf{Pages:}\\ \ref*{TotPages}\vspace*{0.4cm}
    
    \noindent\textbf{Date:}\\ \today\vspace*{0.4cm}\
    
    %\noindent\textbf{\@aauCopiesT:}\\ \@aaucopies
\end{minipage}% This must go next to `\end{minipage}`
\hfill\begin{minipage}[t]{.48\textwidth}
    \vspace*{1cm}
    \noindent\textbf{Abstract:}\vspace*{0.4cm}

    \noindent\fbox{%
        \parbox{\textwidth}{
We present a version of the Mungo language, with the added notion of generic classes. Mungo is an object oriented programming language, that by enforcing a linear typing discipline guarantees that null-derefencing cannot occur. With the introduction of \textit{usages} which are similar to session types, the language allows for protocol specification to ensure that methods will never be called out of order. By extending the notion of a \textit{typestate} with a type parameter we define an object type for generic classes. We present a type system and show that it is a sound approximation of the semantics. Lastly we show a safety result that states that well typed programs never attempts null-dereferencing or deviates from the specified protocols, and ensures protocol completion.
        }
    }
    \end{minipage}
\end{titlepage}
